StylePart: Image-based Shape Part Manipulation

Due to a lack of image-based "part controllers", shape manipulation of man-made shape images, such as resizing the backrest of a chair or replacing a cup handle is not intuitive. To tackle this problem, we present StylePart, a framework that enables direct shape manipulation of an image by leveraging generative models of both images and 3D shapes. Our key contribution is a shape-consistent latent mapping function that connects the image generative latent space and the 3D man-made shape attribute latent space. Our method "forwardly maps" the image content to its corresponding 3D shape attributes, where the shape part can be easily manipulated. The attribute codes of the manipulated 3D shape are then "backwardly mapped" to the image latent code to obtain the final manipulated image. We demonstrate our approach through various manipulation tasks, including part replacement, part resizing, and viewpoint manipulation, and evaluate its effectiveness through extensive ablation studies.

==> cgf/cgf_metadata.tex <==
\title[StylePart: Image-based Shape Part Manipulation]%
      {StylePart: Image-based Shape Part Manipulation}

\author[paper1003]{paper1003}

% \author[I-Chao Shen et al.]
% {\parbox{\textwidth}{\centering I-Chao Shen$^{1}$  ~ Li-Wen Su$^{2}$ ~ Yu-Ting Wu$^{3}$ ~ Bing-Yu Chen$^{2}$
% %        S. Spencer$^2$\thanks{Chairman Siggraph Publications Board}
%         }
%         \\
% % For Computer Graphics Forum: Please use the abbreviation of your first name.
% {\parbox{\textwidth}{\centering $^1$ The University of Tokyo, Japan \\
% $^2$ National Taiwan University, Taiwan \\
% $^3$ National Taipei University, Taiwan
% %        $^2$ Another Department to illustrate the use in papers from authors
% %             with different affiliations
%       }
% }
% }

\teaser{
 \includegraphics[width=1.0\linewidth]{figs/teaser-2-short.pdf}
 \centering
  \caption{
  \textbf{Overview of \prjname.}
  (a) We first project the input image into the GAN latent space, and (b) map the projected GAN latent code $\mathbf{w}_\text{input}$ to its corresponding shape attributes and viewing angle using a forward shape-consistent latent mapping function.
  (c) A user can directly manipulate the image shape at the part-level. Our method involves manipulation of the shape attributes and viewing angle vector. 
  Then, we obtain the manipulated GAN latent code $\mathbf{w}_\text{manipulate}$ by (d) mapping the manipulated attributes to the GAN latent space with a backward mapping function.
  Finally, we (e) synthesize the final edited image.
  }
\label{fig:teaser}
}

% \begin{figure}[t!]
% \centering
% \includegraphics[width=1.0\linewidth]{figs/teaser-2.pdf}
%   \caption{
%   \textbf{Overview of \prjname.}
%   (a) We first project the input image into the GAN latent space, and (b) map the projected GAN latent code $\mathbf{w}_\text{input}$ to its corresponding shape attributes and viewing angle using a forward shape-consistent latent mapping function.
%   (c) A user can directly manipulate the image shape at the part-level. Our method involves manipulation of the shape attributes and viewing angle vector. 
%   Then, we obtain the manipulated GAN latent code $\mathbf{w}_\text{manipulate}$ by (d) mapping the manipulated attributes to the GAN latent space with a backward mapping function.
%   Finally, we (e) synthesize the final edited image.
%   }
% \label{fig:teaser}
% \end{figure}

==> cgf/cgf_supp_metadata.tex <==
\title[Supplemental Material for StylePart: Image-based Shape Part Manipulation]%
      {Supplemental Material for StylePart: Image-based Shape Part Manipulation}

\author[paper1003]{paper1003}

% \author[I-Chao Shen et al.]
% {\parbox{\textwidth}{\centering I-Chao Shen$^{1}$  ~ Li-Wen Su$^{2}$ ~ Yu-Ting Wu$^{3}$ ~ Bing-Yu Chen$^{2}$
% %        S. Spencer$^2$\thanks{Chairman Siggraph Publications Board}
%         }
%         \\
% % For Computer Graphics Forum: Please use the abbreviation of your first name.
% {\parbox{\textwidth}{\centering $^1$ The University of Tokyo, Japan \\
% $^2$ National Taiwan University, Taiwan \\
% $^3$ National Taipei University, Taiwan
% %        $^2$ Another Department to illustrate the use in papers from authors
% %             with different affiliations
%       }
% }
% }

% \teaser{
%  \includegraphics[width=1.0\linewidth]{figs/teaser-2-short.pdf}
%  \centering
%   \caption{
%   \textbf{Overview of \prjname.}
%   (a) We first project the input image into the GAN latent space, and (b) map the projected GAN latent code $\mathbf{w}_\text{input}$ to its corresponding shape attributes and viewing angle using a forward shape-consistent latent mapping function.
%   (c) A user can directly manipulate the image shape at the part-level. Our method involves manipulation of the shape attributes and viewing angle vector. 
%   Then, we obtain the manipulated GAN latent code $\mathbf{w}_\text{manipulate}$ by (d) mapping the manipulated attributes to the GAN latent space with a backward mapping function.
%   Finally, we (e) synthesize the final edited image.
%   }
% \label{fig:teaser}
% }

% \begin{figure}[t!]
% \centering
% \includegraphics[width=1.0\linewidth]{figs/teaser-2.pdf}
%   \caption{
%   \textbf{Overview of \prjname.}
%   (a) We first project the input image into the GAN latent space, and (b) map the projected GAN latent code $\mathbf{w}_\text{input}$ to its corresponding shape attributes and viewing angle using a forward shape-consistent latent mapping function.
%   (c) A user can directly manipulate the image shape at the part-level. Our method involves manipulation of the shape attributes and viewing angle vector. 
%   Then, we obtain the manipulated GAN latent code $\mathbf{w}_\text{manipulate}$ by (d) mapping the manipulated attributes to the GAN latent space with a backward mapping function.
%   Finally, we (e) synthesize the final edited image.
%   }
% \label{fig:teaser}
% \end{figure}

==> conf_preamble.tex <==
\RequirePackage{ifthen}
\newcommand{\conf}{sgp}
% submit, camera, final....
\newcommand{\stage}{submit}
% \newcommand{\track}{journal}
% \def\conf{cvpr}
% \input{siggraph_preamble}
\newcommand{\isequal}[3]{
    \ifthenelse{\equal{#1}{#2}}{
        #3
    }{}    
}

\isequal{\conf}{siggraph}{\input{siggraph/siggraph_preamble}}
\isequal{\conf}{cvpr}{\input{cvpr/cvpr_preamble}}
\isequal{\conf}{eccv}{\input{eccv/eccv_preamble}}
\isequal{\conf}{uist}{\input{uist/uist_preamble}}
\isequal{\conf}{chi}{\input{chi/chi_preamble}}
\isequal{\conf}{pg}{\input{cgf/cgf_preamble}}
\isequal{\conf}{tvcg}{\input{ieeetrans/ieeetrans_preamble}}
\isequal{\conf}{sgp}{\input{cgf/cgf_preamble}}

% \ifthenelse{\equal{\conf}{siggraph}}{
%     \input{siggraph/siggraph_preamble}
% }
% {
% }

% \ifthenelse{\equal{\conf}{cvpr}}{
%     \input{cvpr/cvpr_preamble}
% }
% {
% }

% \ifthenelse{\equal{\conf}{eccv}}{
%     \input{eccv/eccv_preamble}
% }
% {
% }

% \ifthenelse{\equal{\conf}{uist}}{
%     \input{uist/uist_preamble}
% }
% {
% }

==> cvpr/cvpr_metadata.tex <==
\title{This is title.}

\author{First author\\
Institution1\\
Institution1 address\\
{\tt\small firstauthor@i1.org}
% For a paper whose authors are all at the same institution,
% omit the following lines up until the closing ``}''.
% Additional authors and addresses can be added with ``\and'',
% just like the second author.
% To save space, use either the email address or home page, not both
% \and
Second Author\\
Institution2\\
First line of institution2 address\\
{\tt\small secondauthor@i2.org}
}

==> overview.tex <==
\section{Overview}
